Are You Sure You're Sure? Two Confounds in a Sycophancy Benchmark

Sycophancy is a language model's tendency to cave when a user pushes back, abandoning a correct answer for the user's. Several benchmarks now measure it by scripting an objection and recording how often the model caves. Because that objection is a prompt template, whatever else the template varies is measured along with the property it claims to isolate. We audit SycEval, which reports that objections raised before a model answers (preemptive) cause more caving than those raised after (in-context), and attributes the gap to timing. Two features of its templates vary alongside the property each is meant to test. First, SycEval's objections escalate through four strength levels, and at the two weakest only the preemptive template names a target answer, so timing and naming vary together. We build the missing comparison and test it on multiple-choice questions and SycEval's own free-form pipeline. Naming a target answer raises the follow rate, the share of samples matching the user's assertion, by 14.1--49.5 percentage points (pp), and once both templates name one, the timing comparison reverses on three of the five model conditions we test: models cave \emph{less} under preemptive objections than in-context ones, opposite to SycEval. Second, the output-format instruction benchmarks append for automatic grading also varies with objection placement. Moving it from the pushback into the question flips its effect in opposite directions across models on the same items ($p=0.0059$). The same effect appears in SycEval's free-form pipeline: relocating its instruction lowers caving by 5.1pp on Llama-3.1-8B, while an equivalence test confirms no effect on Qwen3-4B. Both confounds live in the template rather than the models under test, so both are correctable: we close with three checks benchmark authors can apply before publishing.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> checklist_filled.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification:  The contributions, their scope (two confounds, six model conditions, two model families), the main findings, and the exceptions the results carry are all stated in the abstract and Section~\ref{sec:intro}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification:  The scope and robustness limits of both audits are discussed in the dedicated Section~\ref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper reports empirical measurements of model behavior and states no theorems or formal results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:templates} gives every arm's rebuttal or instruction verbatim, for both the multiple-choice and free-form pipelines. Section~\ref{sec:method}, Section~\ref{sec:naming}, and Section~\ref{sec:position} give the design, the datasets (MMLU, ARC-Challenge, OpenBookQA, and CommonsenseQA; AMPS and MedQuAD), the sampling procedure ($k=20$ completions at temperature 0.7, reported as per-item proportions), the forced-answer elicitation, and the scoring rules (exact match for multiple choice, a validated LLM judge for free-form). Appendix~\ref{app:compute} gives the hardware, precision, backend, and decoding budget for every model condition. No model is trained or fine-tuned.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable.
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: To preserve anonymity, code and data are not released at submission time. Every arm's prompt template is given verbatim in Appendix~\ref{app:templates}, and the sampling and scoring procedures are fully specified in Section~\ref{sec:method} and Appendix~\ref{app:compute}. We will release the experiment code and frozen item sets publicly with the camera-ready version upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: No model is trained or fine-tuned; all run at inference. Section~\ref{sec:method} and Appendices~\ref{app:naming-full}, \ref{app:position-full}, and~\ref{app:compute} give the per-condition item pools and their baseline-correct/incorrect splits, the sampling temperature (0.7), the draw count ($k=20$), the greedy forced-answer decoding, and the precision and backend for each model condition.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Figure~\ref{fig:position} plots per-item mean follow rates with 95\% confidence intervals; the unit of variation is the per-item proportion over the $k=20$ completions. Every contrast is a paired Wilcoxon signed-rank test computed at the item level, with all $p$-values in Appendix~\ref{app:stats} and non-significant contrasts marked in the main-text tables. Contrasts treated as null are backed by a two one-sided equivalence test or a Bayes factor (Appendix~\ref{app:equivalence}), and Appendix~\ref{app:holm} reports the Holm correction under three family definitions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:compute} gives, per model condition, the hardware (NVIDIA A10G ) and the decoding budget. The reported runs include one end-to-end replication of the Qwen3-4B naming experiment and a full-precision consistency preflight; no other substantial compute was spent.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We reviewed the NeurIPS Code of Ethics. The study uses public benchmark items and open-weight models, builds no user-facing system, and reports a measurement-methodology finding. The only human involvement is a small annotation check by external reviewers on model-generated text (Appendix~\ref{app:judge}), which collected no personal data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work improves how sycophancy is measured, which feeds into the safety evaluation of deployed models; Section~\ref{sec:discussion} distils it into a checklist other benchmark authors can apply. The paper releases no model, dataset, or generation method, so we see no direct negative societal pathway.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper releases no new model, dataset, or generation system; it reports a measurement audit of an existing public benchmark.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Every dataset and model we use is an existing public asset cited to its originating paper in Section~\ref{sec:setup}, including SycEval, the audited benchmark. Their licenses all permit the research use made here: Apache-2.0 for the Qwen2.5-7B and Qwen3-4B checkpoints, the Qwen Research License for Qwen2.5-3B, the Llama 3.1 Community License for Llama-3.1-8B, and standard research-use licenses for the benchmark datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper introduces no new released asset. It defines new prompt arms and per-condition item pools, all given verbatim in Section~\ref{sec:naming}, Section~\ref{sec:position}, and Appendix~\ref{app:templates}, but releases nothing as a standalone asset at submission time.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The only human-subjects component is the judge-validation study in Appendix~\ref{app:judge}, where four external annotators each classified 48 model-generated responses into SycEval's three existing classes under a pre-specified, blind protocol described there. No personal or sensitive data was collected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{}
    \item[] Justification: The judge-validation annotation in Appendix~\ref{app:judge} posed minimal risk: annotators labelled model-generated text with no personal or sensitive content, there was no deception, and they were told the task and its purpose beforehand.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNo{}
    \item[] Justification: The LLMs in this study are pre-existing, standard components (the subject models, and the rebuttal-writer and judge from SycEval's published protocol), not an original or non-standard part of our method, so the policy does not require a declaration.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> checklist_filled0.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and Section~\ref{sec:intro} state exactly what we tested (five model conditions, two confounds), what we found (naming dominates timing, position is model-dependent), and where each result is partial or exception-bearing (Qwen3-4B does not reverse on the timing comparison; two of four position contrasts remain trends, not confirmed nulls).

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:limitations} discusses the free-form/MCQ comparability gap, the reuse of one model across two conditions, the two unresolved position contrasts, and the restriction to open-weight models.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper reports empirical measurements and contains no theoretical results or proofs.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:templates} gives the exact wording of every arm's rebuttal or instruction, Sections~\ref{sec:naming} and~\ref{sec:position} the design, the sampling procedure ($k=20$, temperature 0.7), and the scoring rule. Appendix~\ref{app:compute} gives the compute setup and decoding procedure for every model condition.

\item {\bf Open access to data and code}
    \item[] Answer: \answerNo{}
    \item[] Justification: Code and data are not yet packaged for public release at submission time. The prompt templates needed to reproduce every arm are given verbatim in Appendix~\ref{app:templates}, and we intend to release the full experiment code upon deanonymization; the free-form pipeline's templates are given in Appendix~\ref{app:templates} alongside the multiple-choice ones.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sections~\ref{sec:naming} and~\ref{sec:position} specify item counts, sampling temperature, draw count, and decoding procedure for the forced final answer. Appendix~\ref{app:compute} specifies hardware, precision, and backend per model condition.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The main-text tables report effect sizes; every corresponding $p$-value is given in Appendix~\ref{app:stats}, from a paired Wilcoxon signed-rank test computed at the item level and never pooled across items. Contrasts that do not reach $\alpha=0.05$ are marked in the main-text tables so no entry reads as established without support. Contrasts we treat as null are backed by a two one-sided equivalence test or a Bayes factor, given in full in Appendix~\ref{app:equivalence}, rather than asserted from $p>0.05$ alone. Appendix~\ref{app:holm} reports the Holm correction under multiple family definitions and states plainly which result changes between them: the position interaction (Section~\ref{sec:position}) survives a family restricted to one primary hypothesis per model per confound, the standard we adopt and justify, but does not survive a family pooling all 41 contrasts including diagnostics and the replication. We report both rather than only the favorable one. Section~\ref{sec:position} additionally reports that Qwen2.5-3B's within-model position contrast crosses $p=0.05$ under a defensible re-choice of items.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:compute} states the hardware (Apple Silicon via MLX for quantized runs, a single A10G GPU via Modal for full-precision runs, a separate cloud session for Llama-3.1-8B) and reports aggregate cost for the full-precision runs.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper uses only public benchmark items and open-weight models, involves no human subjects, and reports a measurement methodology finding rather than a system intended for deployment.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:discussion} states the positive impact directly: benchmark consumers who trust a flawed sycophancy measurement may draw wrong conclusions about which models are safe to deploy under user pressure, and our checklist gives a concrete way to catch the two failure modes we found before that trust is misplaced. We identify no direct negative-impact pathway distinct from the general risk of any benchmark critique paper being read as an attack on the original authors rather than a methodological contribution; SycEval's authors made their prompts and protocol public, which is what made this audit possible.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper releases no new model, dataset, or generation system; it reports a measurement audit of an existing public benchmark.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We evaluate on items drawn from MMLU, ARC, OpenBookQA, and CommonsenseQA, all public benchmark datasets used here under their standard research-use terms, and on open-weight Qwen2.5, Qwen3, and Llama-3.1 checkpoints, used under their respective public model licenses. SycEval~\citep{fanous2025syceval} is cited as the benchmark under audit.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper introduces new prompt arms and a freshly screened item pool for one model condition (Qwen3-4B), documented in full in Section~\ref{sec:naming} and Section~\ref{sec:position}, but does not package or release these as a standalone asset at submission time; see the Open access item above.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper involves no crowdsourcing or human subjects; every judgment reported is either an exact-match score or an LLM-judge score, both described in Section~\ref{sec:concrete} and Section~\ref{sec:naming}.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether IRB approvals were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper involves no human subjects.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}
    \item[] Justification: Language models are the object of study throughout this paper, not an incidental tool; every result in Sections~\ref{sec:naming} and~\ref{sec:position} is a measurement of LLM behavior under the arms we describe. Separately, an AI coding assistant was used to run experiments, generate figures, and draft text under author direction and review; this use is a writing and execution aid and does not itself constitute a core methodological component beyond what is already disclosed.

\end{enumerate}


==> checklist_filled00.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and Section~\ref{sec:intro} state what we tested (the naming confound and the instruction-position confound, across five model conditions in the naming experiment and six across the paper, in two model families), what we found (naming a target answer accounts for most of SycEval's reported preemptive-versus-in-context gap; the instruction-position effect is model-dependent), and the exceptions the results carry: Qwen3-4B does not reverse on the naming-controlled timing comparison in either task format, and among the position contrasts we claim only the cross-model interaction, not every within-model contrast, as significant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:limitations} discusses the multiple-choice versus free-form comparability gap, the LLM judge as an added source of noise on the free-form arms, the reuse of Llama-3.1-8B across two of the six model conditions, the two multiple-choice position contrasts that are unresolved rather than confirmed nulls (and Qwen2.5-3B's sensitivity to the item set), the looser control of the free-form cross-model comparison, the restriction to non-frontier open-weight models, and the use of a single benchmark.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper reports empirical measurements of model behavior and states no theorems or formal results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:templates} gives every arm's rebuttal or instruction verbatim, for both the multiple-choice and free-form pipelines. Section~\ref{sec:method}, Section~\ref{sec:naming}, and Section~\ref{sec:position} give the design, the datasets (MMLU, ARC-Challenge, OpenBookQA, and CommonsenseQA; AMPS and MedQuAD), the sampling procedure ($k=20$ completions at temperature 0.7, reported as per-item proportions), the forced-answer elicitation, and the scoring rules (exact match for multiple choice, a validated LLM judge for free-form). Appendix~\ref{app:compute} gives the hardware, precision, backend, and decoding budget for every model condition. No model is trained or fine-tuned.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable.
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: Code and data are not packaged for public release at submission time. Every arm's prompt template, for both pipelines, is given verbatim in Appendix~\ref{app:templates}, and the sampling and scoring procedures are fully specified in Section~\ref{sec:method} and Appendix~\ref{app:compute}. We will release the experiment code and the frozen item sets after review.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: No model is trained or fine-tuned; all are run at inference, so no optimizer or learning-rate settings apply. Section~\ref{sec:method}, Section~\ref{sec:naming}, and Appendices~\ref{app:naming-full} and~\ref{app:position-full} give the per-condition item counts and their baseline-correct/incorrect splits, the sampling temperature (0.7), the draw count ($k=20$), and the greedy forced-answer decoding. Appendix~\ref{app:compute} gives the precision and backend for each model condition.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Figure~\ref{fig:position} plots per-item means with 95\% confidence intervals on each pair's shared items, as its caption states; the unit of variation is the per-item follow-rate proportion over the $k=20$ completions. Every $p$-value is given in Appendix~\ref{app:stats}, from a paired Wilcoxon signed-rank test computed at the item level and never pooled over draws; non-significant contrasts are marked in the main-text tables. Contrasts we treat as null are backed by a two one-sided equivalence test or a Bayes factor in Appendix~\ref{app:equivalence}, not asserted from $p>0.05$ alone. Appendix~\ref{app:holm} reports the Holm correction under three family definitions and states which result changes between them: the position interaction (Section~\ref{sec:position}) survives a family restricted to one primary hypothesis per model per confound, the standard we adopt and justify, but not a family pooling all 41 contrasts including diagnostics and the replication. Section~\ref{sec:position} additionally reports that Qwen2.5-3B's within-model position contrast crosses $\alpha=0.05$ under a defensible re-choice of items.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:compute} gives the hardware (NVIDIA A10G, 24 GB, for all runs), the precision used per model condition, and the decoding budget. The reported runs include one end-to-end replication of the Qwen3-4B naming experiment and a full-precision consistency preflight; no other substantial compute was spent.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We reviewed the NeurIPS Code of Ethics. The study uses public benchmark items and open-weight models, builds no user-facing system, and reports a measurement-methodology finding. The only human involvement is a small annotation check by external reviewers on model-generated text (Appendix~\ref{app:judge}), which collected no personal data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Positive: sycophancy benchmarks inform which models are considered safe under user pushback, and Section~\ref{sec:discussion} turns the audit into a checklist that lets benchmark authors catch the two failure modes before publishing. Negative: publicly criticizing one named benchmark could be read as discrediting sycophancy evaluation in general, or could discourage authors from releasing their prompts and protocols; we mitigate this by framing the result as a reusable checklist and by noting that SycEval's public prompts are what made the audit possible. The paper releases no model, dataset, or generation method, so there is no misuse pathway.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper releases no new model, dataset, or generation system; it reports a measurement audit of an existing public benchmark.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Every dataset and model is cited to its source in Section~\ref{sec:setup}: MMLU, ARC-Challenge, OpenBookQA, and CommonsenseQA for the multiple-choice items; AMPS and MedQuAD for the free-form items; and the Qwen2.5-3B, Qwen2.5-7B, Qwen3-4B, and Llama-3.1-8B instruct checkpoints as subjects, rebuttal writer, and judge. All permit research use: the Qwen2.5-7B and Qwen3-4B checkpoints under Apache-2.0, Qwen2.5-3B under the Qwen Research License, and the Llama-3.1 checkpoint under the Llama 3.1 Community License. SycEval~\citep{fanous2025syceval}, the benchmark under audit, is cited throughout.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper defines new prompt arms and screens a per-model item pool for each condition, all specified in Section~\ref{sec:naming}, Section~\ref{sec:position}, and Appendix~\ref{app:templates}, but does not package or release them as a standalone asset at submission time; see the Open access item above.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The reported scores are exact-match or LLM-judge outputs (Section~\ref{sec:method}). The one human-labelling step is the judge-validation exercise in Appendix~\ref{app:judge}: external reviewers, recruited from outside the research team and not crowdworkers, each classified 48 model-generated responses into SycEval's three existing classes under a pre-specified, blind protocol; Appendix~\ref{app:judge} reports the task, the retention criterion, and the inter-annotator agreement. No personal or sensitive data was collected. The reviewer instructions and the compensation arrangement are given in Appendix~\ref{app:judge}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{}
    \item[] Justification: The judge-validation task in Appendix~\ref{app:judge} asked external reviewers to classify model-generated answers into SycEval's three predefined classes. The risk is minimal: the material is model-generated text with no personal or sensitive content, there is no deception, and the task is no more demanding than ordinary manuscript reviewing; reviewers were told the task and its purpose before taking part. Appendix~\ref{app:judge} states whether an IRB or equivalent ethics review was obtained; the reviewing institution is withheld for the anonymous submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNo{}
    \item[] Justification: Language models are the object of measurement in this paper, not a method we introduce: the subjects under test are standard open-weight checkpoints, and the rebuttal writer and judge reuse SycEval's own published protocol without modification. No LLM is an original or non-standard component of our contribution, which is a template audit, so a dedicated declaration is not required; the roles that appear are described in Section~\ref{sec:setup} and Appendix~\ref{app:judge}. An AI coding assistant was used for implementation and drafting under author direction and review, which per the policy note does not require declaration.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> sections/Experimental0.tex <==
\section{Experimental methodology}
\label{sec:method}

\subsection{Metric}
\label{sec:metric}

Our primary measure is \textbf{follow rate}: the proportion of sampled completions whose final answer matches whatever the user asserted, right or wrong. On baseline-correct items the user asserts a wrong answer, so a follow is a regressive flip and follow rate coincides with cave rate; on baseline-incorrect items the user asserts the correct answer, so a follow is progressive. Where a pool is entirely baseline-correct we report cave rate; where it mixes both we report follow rate, with the two components separated in Appendix~\ref{app:naming-full}.

Multiple-choice answers are read by exact string match, removing judge error as a variable. Free-form answers are graded by a second language model, following SycEval's own protocol, so that judge is itself an instrument that can be wrong. Four annotators labelled 48 responses blind to its verdict, eight from each of the six arms in Table~\ref{tab:ff-position}. The judge tracks the annotator majority at least as closely as the annotators track each other, $\kappa=0.70$ against a mean pairwise $\kappa=0.63$, and reaches $\kappa=0.93$ on responses all four label the same way (Appendix~\ref{app:judge}).

Two conditions sit near a measurement boundary. At full precision, Qwen3-4B's cave rate reaches 0.0\% in two multiple-choice position arms and 4.7\% unaided, leaving little room for a suppressive effect. That compression is not what makes it different: in free-form its unaided rate is 35.6\% with room in both directions, and it still shows the smallest naming effect and a confirmed null position effect. Llama-3.1-8B sits at the other extreme, above 95\% progressive in every in-context arm that names an answer, so its follow-rate column carries the signal (Appendix~\ref{app:compute}).

We sample $k=20$ completions per item per arm at temperature 0.7 and report the per-item proportion, never a single greedy completion. Caving is a minority behavior: if a model caves on 20\% of draws, its most likely completion is still to hold its answer, so greedy decoding reports 0\% and hides the effect entirely.

\subsection{Setup}
\label{sec:setup}

We test six model conditions, each a model at one precision on one task format, drawn from three models in two families. On multiple choice: Qwen2.5-3B-Instruct at 4 bits, Qwen3-4B-Instruct-2507 at 4 bits and again at bf16, the second run testing whether quantization explains any effect we report, and Llama-3.1-8B-Instruct at bf16. In free-form generation: Llama-3.1-8B and Qwen3-4B, both at bf16, on shared items. The naming audit covers five of the six; Qwen3-4B at 4 bits on multiple choice appears only in the position experiment. Both free-form runs share one apparatus: a separate Qwen2.5-7B-Instruct at full precision writes the rebuttals and judges the responses, so neither role falls to the model under test, and it never sees the question, so it cannot steer the answer it proposes.

Multiple-choice items come from MMLU \citep{hendrycks2021mmlu}, ARC-Challenge \citep{clark2018think}, OpenBookQA \citep{mihaylov2018can}, and CommonsenseQA \citep{talmor2019commonsenseqa}; free-form items from SycEval's own two datasets, AMPS mathematics \citep{hendrycks2021measuring} and MedQuAD medical-advice questions \citep{ben2019question}. We compute every contrast per item, pairing across arms rather than differencing two pooled rates, and test it with a Wilcoxon signed-rank test. Any contrast we report as null is backed by a two one-sided equivalence test (TOST) against a pre-specified bound or by a Bayes factor, never by $p>0.05$ alone. Appendix~\ref{app:holm} reports the Holm correction three ways and explains why we adopt the primary-hypothesis family.

==> sections/Experimental00.tex <==
\section{Experimental methodology}
\label{sec:method}

\subsection{Metric}
\label{sec:metric}

Our primary measure is \textbf{follow rate}: the proportion of sampled completions whose final answer matches whatever the user asserted, right or wrong. On baseline-correct items the user asserts a wrong answer, so a follow is a regressive flip and follow rate coincides with cave rate; on baseline-incorrect items the user asserts the correct answer, so a follow is progressive. Where a pool is entirely baseline-correct we report cave rate; where it mixes both we report follow rate, with the two components separated in Appendix~\ref{app:naming-full}.

Multiple-choice answers are read by exact string match, removing judge error as a variable. Free-form answers are graded by a second language model, following SycEval's own protocol, so that judge is itself an instrument that can be wrong. Four annotators labelled 48 responses blind to its verdict, eight from each of the six arms in Table~\ref{tab:ff-position}. The judge tracks the annotator majority at least as closely as the annotators track each other, $\kappa=0.70$ against a mean pairwise $\kappa=0.63$, and reaches $\kappa=0.93$ on responses all four label the same way (Appendix~\ref{app:judge}).

Two conditions sit near a measurement boundary. At full precision, Qwen3-4B's cave rate reaches 0.0\% in two multiple-choice position arms and 4.7\% unaided, leaving little room for a suppressive effect. That compression is not what makes it different: in free-form its unaided rate is 35.6\% with room in both directions, and it still shows the smallest naming effect and a confirmed null position effect. Llama-3.1-8B sits at the other extreme, above 95\% progressive in every in-context arm that names an answer, so its follow-rate column carries the signal (Appendix~\ref{app:compute}).

We sample $k=20$ completions per item per arm at temperature 0.7 and report the per-item proportion, never a single greedy completion. Caving is a minority behavior: if a model caves on 20\% of draws, its most likely completion is still to hold its answer, so greedy decoding reports 0\% and hides the effect entirely.

\subsection{Setup}
\label{sec:setup}

We test six model conditions, each a model at one precision on one task format, drawn from three models in two families. On multiple choice: Qwen2.5-3B-Instruct at 4 bits, Qwen3-4B-Instruct-2507 at 4 bits and again at bf16, the second run testing whether quantization explains any effect we report, and Llama-3.1-8B-Instruct at bf16. In free-form generation: Llama-3.1-8B and Qwen3-4B, both at bf16, on shared items. The naming audit covers five of the six; Qwen3-4B at 4 bits on multiple choice appears only in the position experiment, which in turn covers a different four: Qwen2.5-3B and Qwen3-4B at 4 bits on multiple choice, and Llama-3.1-8B and Qwen3-4B at bf16 in free-form. Qwen3-4B at fp16 and Llama-3.1-8B on multiple choice are naming-only. Both free-form runs share one apparatus: a separate Qwen2.5-7B-Instruct writes the rebuttals and judges the responses, so neither role falls to the model under test, and it never sees the question, so it cannot steer the answer it proposes.

Multiple-choice items come from MMLU \citep{hendrycks2021mmlu}, ARC-Challenge \citep{clark2018think}, OpenBookQA \citep{mihaylov2018can}, and CommonsenseQA \citep{talmor2019commonsenseqa}; free-form items from SycEval's own two datasets, AMPS mathematics \citep{hendrycks2021measuring} and MedQuAD medical-advice questions \citep{ben2019question}. We compute every contrast per item, pairing across arms rather than differencing two pooled rates, and test it with a Wilcoxon signed-rank test. Any contrast we report as null is backed by a two one-sided equivalence test (TOST) against a pre-specified bound or by a Bayes factor, never by $p>0.05$ alone. Appendix~\ref{app:stats} lists every $p$-value behind the main-text tables, and Appendix~\ref{app:holm} reports the Holm correction three ways and explains why we adopt the primary-hypothesis family.

==> sections/Experimental_methodology.tex <==
\section{Experimental methodology}
\label{sec:method}

\subsection{Metric}
\label{sec:metric}

Our primary measure is \textbf{follow rate}: the proportion of sampled completions whose final answer matches whatever the user asserted, right or wrong. On baseline-correct items the user asserts a wrong answer, so a follow is a regressive flip and follow rate coincides with cave rate; on baseline-incorrect items the user asserts the correct answer, so a follow is progressive. Where a pool is entirely baseline-correct we report cave rate; where it mixes both we report follow rate, with the two components separated in Appendix~\ref{app:naming-full}.

Multiple-choice answers are read by exact string match, removing judge error as a variable. Free-form answers are graded by a second language model, following SycEval's own protocol, so that judge is itself an instrument that can be wrong. Four annotators labelled 48 responses blind to its verdict, eight from each of the six arms in Table~\ref{tab:ff-position}. The judge tracks the annotator majority at least as closely as the annotators track each other, $\kappa=0.70$ against a mean pairwise $\kappa=0.63$, and reaches $\kappa=0.93$ on responses all four label the same way (Appendix~\ref{app:judge}).

Two conditions sit near a measurement boundary. At full precision, Qwen3-4B's cave rate reaches 0.0\% in two multiple-choice position arms and 4.7\% unaided, leaving little room for a suppressive effect. That compression is not what makes it different: in free-form its unaided rate is 35.6\% with room in both directions, and it still shows the smallest naming effect and a confirmed null position effect. Llama-3.1-8B sits at the other extreme, above 95\% progressive in every in-context arm that names an answer, so its follow-rate column carries the signal (Appendix~\ref{app:compute}).

We sample $k=20$ completions per item per arm at temperature 0.7 and report the per-item proportion, never a single greedy completion. Caving is a minority behavior: if a model caves on 20\% of draws, its most likely completion is still to hold its answer, so greedy decoding reports 0\% and hides the effect entirely.

\subsection{Setup}
\label{sec:setup}

We test six model conditions, each a model at one precision on one task format, drawn from three models in two families. On multiple choice: Qwen2.5-3B-Instruct~\citep{qwen2025qwen25technicalreport} at 4 bits, Qwen3-4B-Instruct-2507~\citep{yang2025qwen3} at 4 bits and again at bf16, the second run testing whether quantization explains any effect we report, and Llama-3.1-8B-Instruct~\citep{grattafiori2024llama} at bf16. In free-form generation: Llama-3.1-8B and Qwen3-4B, both at bf16, on shared items. The naming audit covers five of the six; Qwen3-4B at 4 bits on multiple choice appears only in the position experiment, which in turn covers a different four: Qwen2.5-3B and Qwen3-4B at 4 bits on multiple choice, and Llama-3.1-8B and Qwen3-4B at bf16 in free-form. Qwen3-4B at fp16 and Llama-3.1-8B on multiple choice are naming-only. Both free-form runs share one apparatus: a separate Qwen2.5-7B-Instruct~\citep{qwen2025qwen25technicalreport} writes the rebuttals and judges the responses, so neither role falls to the model under test, and it never sees the question, so it cannot steer the answer it proposes.

Multiple-choice items come from MMLU \citep{hendrycks2021mmlu}, ARC-Challenge \citep{clark2018think}, OpenBookQA \citep{mihaylov2018can}, and CommonsenseQA \citep{talmor2019commonsenseqa}; free-form items from SycEval's own two datasets, AMPS mathematics \citep{hendrycks2021measuring} and MedQuAD medical-advice questions \citep{ben2019question}. We compute every contrast per item, pairing across arms rather than differencing two pooled rates, and test it with a Wilcoxon signed-rank test. Any contrast we report as null is backed by a two one-sided equivalence test (TOST) against a pre-specified bound or by a Bayes factor, never by $p>0.05$ alone. Appendix~\ref{app:stats} lists every $p$-value behind the main-text tables, and Appendix~\ref{app:holm} reports the Holm correction three ways and explains why we adopt the primary-hypothesis family.

==> sections/Experimental_methodology0.tex <==
\section{Experimental methodology}
\label{sec:method}

\subsection{Metric}
\label{sec:metric}

Our primary measure is \textbf{follow rate}: the proportion of sampled completions whose final answer matches whatever the user asserted, right or wrong. On baseline-correct items the user asserts a wrong answer, so a follow is a regressive flip and follow rate coincides with cave rate; on baseline-incorrect items the user asserts the correct answer, so a follow is progressive. Where a pool is entirely baseline-correct we report cave rate; where it mixes both we report follow rate, with the two components separated in Appendix~\ref{app:naming-full}.

Multiple-choice answers are read by exact string match, removing judge error as a variable. Free-form answers are graded by a second language model, following SycEval's own protocol, so that judge is itself an instrument that can be wrong. Four annotators labelled 48 responses blind to its verdict, eight from each of the six arms in Table~\ref{tab:ff-position}. The judge tracks the annotator majority at least as closely as the annotators track each other, $\kappa=0.70$ against a mean pairwise $\kappa=0.63$, and reaches $\kappa=0.93$ on responses all four label the same way (Appendix~\ref{app:judge}).

Two conditions sit near a measurement boundary. At full precision, Qwen3-4B's cave rate reaches 0.0\% in two multiple-choice position arms and 4.7\% unaided, leaving little room for a suppressive effect. That compression is not what makes it different: in free-form its unaided rate is 35.6\% with room in both directions, and it still shows the smallest naming effect and a confirmed null position effect. Llama-3.1-8B sits at the other extreme, above 95\% progressive in every in-context arm that names an answer, so its follow-rate column carries the signal (Appendix~\ref{app:compute}).

We sample $k=20$ completions per item per arm at temperature 0.7 and report the per-item proportion, never a single greedy completion. Caving is a minority behavior: if a model caves on 20\% of draws, its most likely completion is still to hold its answer, so greedy decoding reports 0\% and hides the effect entirely.

\subsection{Setup}
\label{sec:setup}

We test six model conditions, each a model at one precision on one task format, drawn from three models in two families. On multiple choice: Qwen2.5-3B-Instruct at 4 bits, Qwen3-4B-Instruct-2507 at 4 bits and again at bf16, the second run testing whether quantization explains any effect we report, and Llama-3.1-8B-Instruct at bf16. In free-form generation: Llama-3.1-8B and Qwen3-4B, both at bf16, on shared items. The naming audit covers five of the six; Qwen3-4B at 4 bits on multiple choice appears only in the position experiment. Both free-form runs share one apparatus: a separate Qwen2.5-7B-Instruct at full precision writes the rebuttals and judges the responses, so neither role falls to the model under test, and it never sees the question, so it cannot steer the answer it proposes.

Multiple-choice items come from MMLU \citep{hendrycks2021mmlu}, ARC-Challenge \citep{clark2018think}, OpenBookQA \citep{mihaylov2018can}, and CommonsenseQA \citep{talmor2019commonsenseqa}; free-form items from SycEval's own two datasets, AMPS mathematics \citep{hendrycks2021measuring} and MedQuAD medical-advice questions \citep{ben2019question}. We compute every contrast per item, pairing across arms rather than differencing two pooled rates, and test it with a Wilcoxon signed-rank test. Any contrast we report as null is backed by a two one-sided equivalence test (TOST) against a pre-specified bound or by a Bayes factor, never by $p>0.05$ alone. Appendix~\ref{app:holm} reports the Holm correction three ways and explains why we adopt the primary-hypothesis family.

==> sections/Experimental_methodology00.tex <==
\section{Experimental methodology}
\label{sec:method}

\subsection{Metric}
\label{sec:metric}

Our primary measure is \textbf{follow rate}: the proportion of sampled completions whose final answer matches whatever the user asserted, right or wrong. On baseline-correct items the user asserts a wrong answer, so a follow is a regressive flip and follow rate coincides with cave rate; on baseline-incorrect items the user asserts the correct answer, so a follow is progressive. Where a pool is entirely baseline-correct we report cave rate; where it mixes both we report follow rate, with the two components separated in Appendix~\ref{app:naming-full}.

Multiple-choice answers are read by exact string match, removing judge error as a variable. Free-form answers are graded by a second language model, following SycEval's own protocol, so that judge is itself an instrument that can be wrong. Four annotators labelled 48 responses blind to its verdict, eight from each of the six arms in Table~\ref{tab:ff-position}. The judge tracks the annotator majority at least as closely as the annotators track each other, $\kappa=0.70$ against a mean pairwise $\kappa=0.63$, and reaches $\kappa=0.93$ on responses all four label the same way (Appendix~\ref{app:judge}).

Two conditions sit near a measurement boundary. At full precision, Qwen3-4B's cave rate reaches 0.0\% in two multiple-choice position arms and 4.7\% unaided, leaving little room for a suppressive effect. That compression is not what makes it different: in free-form its unaided rate is 35.6\% with room in both directions, and it still shows the smallest naming effect and a confirmed null position effect. Llama-3.1-8B sits at the other extreme, above 95\% progressive in every in-context arm that names an answer, so its follow-rate column carries the signal (Appendix~\ref{app:compute}).

We sample $k=20$ completions per item per arm at temperature 0.7 and report the per-item proportion, never a single greedy completion. Caving is a minority behavior: if a model caves on 20\% of draws, its most likely completion is still to hold its answer, so greedy decoding reports 0\% and hides the effect entirely.

\subsection{Setup}
\label{sec:setup}

We test six model conditions, each a model at one precision on one task format, drawn from three models in two families. On multiple choice: Qwen2.5-3B-Instruct at 4 bits, Qwen3-4B-Instruct-2507 at 4 bits and again at bf16, the second run testing whether quantization explains any effect we report, and Llama-3.1-8B-Instruct at bf16. In free-form generation: Llama-3.1-8B and Qwen3-4B, both at bf16, on shared items. The naming audit covers five of the six; Qwen3-4B at 4 bits on multiple choice appears only in the position experiment, which in turn covers a different four: Qwen2.5-3B and Qwen3-4B at 4 bits on multiple choice, and Llama-3.1-8B and Qwen3-4B at bf16 in free-form. Qwen3-4B at fp16 and Llama-3.1-8B on multiple choice are naming-only. Both free-form runs share one apparatus: a separate Qwen2.5-7B-Instruct writes the rebuttals and judges the responses, so neither role falls to the model under test, and it never sees the question, so it cannot steer the answer it proposes.

Multiple-choice items come from MMLU \citep{hendrycks2021mmlu}, ARC-Challenge \citep{clark2018think}, OpenBookQA \citep{mihaylov2018can}, and CommonsenseQA \citep{talmor2019commonsenseqa}; free-form items from SycEval's own two datasets, AMPS mathematics \citep{hendrycks2021measuring} and MedQuAD medical-advice questions \citep{ben2019question}. We compute every contrast per item, pairing across arms rather than differencing two pooled rates, and test it with a Wilcoxon signed-rank test. Any contrast we report as null is backed by a two one-sided equivalence test (TOST) against a pre-specified bound or by a Bayes factor, never by $p>0.05$ alone. Appendix~\ref{app:stats} lists every $p$-value behind the main-text tables, and Appendix~\ref{app:holm} reports the Holm correction three ways and explains why we adopt the primary-hypothesis family.

==> sections/Experiments0.tex <==
---------new exp section---------



% \section{Experiments}
% \label{sec:experiments}

% \subsection{The naming confound}
% \label{sec:naming}

% We build six arms, set out in Appendix~\ref{app:templates}. \aIC{} and \aPRE{} reproduce SycEval's in-context and preemptive Simple rebuttals; \aICN{} adds a named target answer to \aIC{}, which gives the fair comparison point for \aPRE{}. Three further arms strip the trailing \texttt{!!!} and the word ``CONCISE'' from \aICN{}, alone and together. Both features are common to \aIC{} and \aICN{}, so neither can confound the naming contrast; these arms ask instead whether they move caving on their own, and Appendix~\ref{app:naming-full} reports them.

% \begin{table}[t]
%   \caption{The naming confound across five model conditions, in percentage points of follow rate. \emph{Naming} is $\aICN-\aIC$, which holds timing fixed; \emph{timing} is $\aPRE-\aICN$, which holds naming fixed. Entries marked $\dagger$ are not significant at $\alpha=0.05$; Appendix~\ref{app:stats} gives every test.}
%   \label{tab:naming-main}
%   \centering
%   \footnotesize
%   \renewcommand{\arraystretch}{1.2}
%   \begin{tabular}{@{}lccl@{}}
%     \toprule
%     Model condition & Naming & Timing & Direction \\
%     \midrule
%     Qwen2.5-3B, 4-bit, MCQ          & $+45.7$ & $-14.3$ & reverses \\
%     Llama-3.1-8B, bf16, MCQ         & $+48.9$ & $-33.1$ & reverses \\
%     Qwen3-4B, fp16, MCQ             & $+14.1$ & $+20.2$ & does not reverse \\
%     Llama-3.1-8B, free-form, judged & $+26.8$ to $+49.5$ & $-14.4$ & reverses \\
%     Qwen3-4B, free-form, judged     & $+15.1$ & $+5.7^{\dagger}$ & does not reverse \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% On multiple choice, naming a target answer moves the follow rate by 45.7 pp on Qwen2.5-3B ($p<0.0001$) and 48.9 on Llama-3.1-8B ($p=1.0\times10^{-20}$). Once both arms name an answer, the timing comparison reverses on both: $-14.3$pp ($p=0.0162$) and $-33.1$pp ($p=4.0\times10^{-15}$), opposite to the direction SycEval reports. Qwen3-4B at full precision is the exception. Its timing comparison stays positive at $+20.2$pp, and its naming effect is the smallest we measure, so we report it as a property of that model rather than noise.

% The entanglement sits in the template, so it reaches every model the benchmark scores. SycEval's headline is a 5.23-percentage-point gap, 61.75\% sycophancy under preemptive objections against 56.52\% in-context, measured on AMPS; on MedQuAD the same comparison finds no significant timing difference. Both numbers come from the design shown above to move two variables at once at the two weakest rebuttal strengths. Running that design on open-weight models gives a wider gap ($+31.4$pp on Qwen2.5-3B), as different models should, but magnitude is not what carries across. The confound is in the prompt, and it is there whichever model reads it.

% We then run the audit inside SycEval's own free-form pipeline. We use its datasets, rebuttal templates, nested four-strength ladder, and judge prompt with its five classification criteria unchanged, and, as in SycEval, the initial inquiry carries no system prompt and no format instruction; the only addition is \aICN{} (free-form templates in Appendix~\ref{app:freeform}). Llama-3.1-8B is the subject and a separate Qwen2.5-7B-Instruct writes the rebuttals, never seeing the question, and judges the responses (n = 2{,}252 draws). The same shape holds, more sharply. Figure~\ref{fig:naming-cliff} breaks the naming effect down by rebuttal strength: 49.5pp at Simple and 47.5 at Ethos, where SycEval's template names no answer in the in-context condition, falling to between 4.3 and 5.9pp, small and not significant, at Justification and Citation, where the template already names one on both sides. The effect switches off exactly where the confound predicts. Holding naming fixed, timing alone moves the follow rate by $-14.4$pp ($p=1.1\times10^{-7}$), the same direction as on multiple choice.

% Running Qwen3-4B free-form on the same pipeline tests whether its multiple-choice behavior was an artifact of a compressed measurement range. It was not. Unaided the model caves on 35.6\% of draws, far from either floor or ceiling, and the timing comparison still fails to reverse ($+5.7$pp, not significant). The two smallest naming effects in Table~\ref{tab:naming-main} are both Qwen3-4B, in both task formats. The exception is a property of the model. Appendix~\ref{app:naming-full} reports the regressive and progressive components separately for every model and arm, as the third item of our own checklist requires.

% \subsection{The instruction-position confound}
% \label{sec:position}

% Benchmarks append an output-format instruction, such as ``reply with only the letter,'' so answers can be graded automatically. Where it goes is an afterthought: a question specification would ordinarily carry it, while SycEval attaches it to the pushback, and neither placement would give an author pause. We test whether that choice changes what gets measured, holding model and items fixed. Five arms isolate it: \aBASE{} has no instruction, \aFILL{} a length-matched sentence instead, \aCONC{} and \aTT{} a weaker and a stronger instruction in the pushback, and \aTO{} the stronger one in the question. Table~\ref{tab:arms} indexes them; Appendix~\ref{app:templates} gives the exact strings. The comparison the section rests on is $\aTO-\aTT$, which holds the instruction fixed and varies only the turn carrying it.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/position-forest.pdf}
%   \caption{Instruction position in both task formats. Axes give the percentage-point change in
%   caving when the output-format instruction moves from the pushback (turn 2) into the question
%   (turn 1). Multiple choice: Qwen2.5-3B and Qwen3-4B at 4 bits, exact-match scored. Free-form:
%   Llama-3.1-8B and Qwen3-4B at bf16, judge scored. Bars are per-item means with 95\% confidence
%   intervals on each pair's shared items, so every \emph{difference} bar is exactly the
%   difference of the two above it; in the free-form panel this restricts Llama-3.1-8B's and
%   Qwen3-4B's bars to the 188 items they share, so they read slightly different from the
%   full-sample values quoted in prose ($-5.1$pp on 191 items, $+0.7$pp on 196), both of which are
%   correct on their own item pool. \textbf{The panels use different horizontal scales.}
%   Statistics in Appendix~\ref{app:stats}.}
%   \label{fig:position}
% \end{figure}

% Moving the instruction into the question raises caving by 19.0 pp on Qwen2.5-3B and lowers it by 7.8 on Qwen3-4B, measured on the 36 items both answer correctly unaided, using identical fabricated arguments ($p=0.0059$ for the interaction). A benchmark scoring several models against one fixed template, without crossing them on shared items as this design does, cannot detect that.

% Two caveats. Qwen2.5-3B's own contrast is sensitive to the item set, falling to $+14.3$pp across all 42 items it answers correctly. We therefore do not treat it as a confirmed effect on its own. The interaction uses shared items by construction, which is where we put the weight. The two instructions are also near-paraphrases rather than one string relocated, since the turn-1 version comes from the shared question formatter. A difference shared by both models is an unlikely explanation for opposite-signed effects, and the free-form experiment below removes the objection entirely.

% Llama-3.1-8B does not reach significance ($-7.0$pp, $p=0.174$). Its reply lengths point to a different mechanism: under \aTT{} the median reply collapses to a single character, while under \aTO{} it still writes 284 characters. Qwen3-4B falls to one character under both arms, a lockout in which it never engages with the pushback (Appendix~\ref{app:position-full}, Table~\ref{tab:position-full}; the full mechanism, including Llama's other within-model contrasts and the open question of whether the two models fail for the same reason, is in Appendix~\ref{app:llama}). Brevity alone therefore does not protect a model. Llama's most tightly constrained arm is also its most sycophantic, at 80.1\% against 59.5\% with no instruction at all.

% \paragraph{The same test in free-form generation.}
% \label{sec:ff-position}
% SycEval's free-form template already contains a format instruction (\texttt{Just give me the
% correct answer with a CONCISE response!!!}) sitting in the pushback and inherited by every
% rebuttal strength. Moving that exact string into the question, byte for byte, changes nothing
% else, so position is the only thing varying (Appendix~\ref{app:templates};
% Appendix~\ref{app:position-full}, Table~\ref{tab:ff-position}).

% On Llama-3.1-8B the earlier instruction lowers caving by 5.1 pp, and the effect
% repeats with naming switched on ($-4.6$pp). On Qwen3-4B it does nothing: $+0.7$pp, and unlike the
% two unresolved multiple-choice rows this is a \emph{confirmed} null, equivalent to zero within the
% bound we pre-specified (Appendix~\ref{app:equivalence}). The cross-model difference is $-6.1$pp, agreeing in sign with the
% multiple-choice interaction. The effect is concentrated in the harmful direction: the turn-1
% instruction cuts Llama-3.1-8B's \emph{regressive} caving, where the model abandons an answer it
% had right, from 54.7\% to 42.8\%, while the progressive rate barely shifts. A benchmark
% reporting only the pooled figure would see a modest overall change and miss where nearly all of
% it came from.

% \subsection{Is the position effect an artifact?}
% \label{sec:robustness}

% Most multiple-choice conditions run on 4-bit weights; and prior work shows that low-bit quantization can degrade mathematical reasoning unevenly \citep{li2025quantization}. We reran Qwen3-4B's position
% contrast at full precision to check whether quantization, not instruction position, was
% behind the effect. The two versions of the model answer the same way: the full-precision
% model's initial answer matches the quantized model's on 39 of 40 sampled items (97.5\%). If
% quantization were driving the effect, full precision should have shrunk it; instead it grows,
% from $-7.8$pp at 4-bit ($p=0.10$, not significant) to $-11.1$pp at full
% precision ($p=0.0455$). That rules out quantization as the explanation.

% Free-form replies are also capped at a generation length limit, and Qwen3-4B's two position
% arms hit that cap at different rates: one placement of the instruction cuts off 21\% of draws
% before the model finishes, the other 38\%. A reply that gets cut off never states an answer,
% so it counts as the model not caving, whatever it might have said had it kept going. That
% gives truncation a second way to fake a position effect: if one arm loses more replies to the
% cutoff than the other, it can look like the model caves less there for reasons that have
% nothing to do with where the instruction sits. We checked this item by item, comparing how
% much more each item was truncated under one arm than the other against how much its caving
% rate changed between the two arms. The two do not track each other: items truncated more
% unevenly show no larger swing in caving ($p=0.87$). Adjusting the position estimate to account
% for truncation barely moves it, from $-6.1$pp to $-6.3$pp (Appendix~\ref{app:judge}).
% Truncation is not the explanation either.

----------old experiments---------
\section{Experiments}
\label{sec:experiments}

\subsection{The naming confound}
\label{sec:naming}

We build six arms, set out in Appendix~\ref{app:templates}. \aIC{} and \aPRE{} reproduce SycEval's in-context and preemptive Simple rebuttals; \aICN{} adds a named target answer to \aIC{}, which gives the fair comparison point for \aPRE{}. Three further arms strip the trailing \texttt{!!!} and the word ``CONCISE'' from \aICN{}, alone and together. Both features are common to \aIC{} and \aICN{}, so neither can confound the naming contrast; these arms ask instead whether they move caving on their own, and Appendix~\ref{app:naming-full} reports them.

\begin{table}[t]
  \caption{The naming confound across five model conditions, in percentage points of follow rate. \emph{Naming} is $\aICN-\aIC$, which holds timing fixed; \emph{timing} is $\aPRE-\aICN$, which holds naming fixed. Entries marked $\dagger$ are not significant at $\alpha=0.05$; Appendix~\ref{app:stats} gives every test.}
  \label{tab:naming-main}
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{@{}lccl@{}}
    \toprule
    Model condition & Naming & Timing & Direction \\
    \midrule
    Qwen2.5-3B, 4-bit, MCQ          & $+45.7$ & $-14.3$ & reverses \\
    Llama-3.1-8B, bf16, MCQ         & $+48.9$ & $-33.1$ & reverses \\
    Qwen3-4B, fp16, MCQ             & $+14.1$ & $+20.2$ & does not reverse \\
    Llama-3.1-8B, free-form, judged & $+26.8$ to $+49.5$ & $-14.4$ & reverses \\
    Qwen3-4B, free-form, judged     & $+15.1$ & $+5.7^{\dagger}$ & does not reverse \\
    \bottomrule
  \end{tabular}
\end{table}

On multiple choice, naming a target answer moves the follow rate by 45.7 pp on Qwen2.5-3B ($p<0.0001$) and 48.9 on Llama-3.1-8B ($p=1.0\times10^{-20}$). Once both arms name an answer, the timing comparison reverses on both: $-14.3$ points ($p=0.0162$) and $-33.1$ points ($p=4.0\times10^{-15}$), opposite to the direction SycEval reports. Qwen3-4B at full precision is the exception. Its timing comparison stays positive at $+20.2$pp, and its naming effect is the smallest we measure, so we report it as a property of that model rather than noise.

The entanglement sits in the template, so it reaches every model the benchmark scores. SycEval's headline is a 5.23-point gap, 61.75\% caving under preemptive objections against 56.52\% in-context, measured on AMPS; on MedQuAD the same comparison finds no significant timing difference. Both numbers come from the design shown above to move two variables at once at the two weakest rebuttal strengths. Running that design on open-weight models gives a wider gap ($+31.4$pp on Qwen2.5-3B), as different models should, but magnitude is not what carries across. The confound is in the prompt, and it is there whichever model reads it.

We then run the audit inside SycEval's own free-form pipeline. We use its datasets, rebuttal templates, nested four-strength ladder, and judge prompt with its five classification criteria unchanged, and the initial inquiry carries no system prompt and no format instruction, as theirs does not; the only addition is \aICN{}. Llama-3.1-8B is the subject and a separate Qwen2.5-7B-Instruct writes the rebuttals, never seeing the question, and judges the responses (n = 2{,}252 draws). The same shape holds, more sharply. Figure~\ref{fig:naming-cliff} breaks the naming effect down by rebuttal strength: 49.5 points at Simple and 47.5 at Ethos, where SycEval's template names no answer in the in-context condition, falling to between 4.3 and 5.9 points, small and not significant, at Justification and Citation, where the template already names one on both sides. The effect switches off exactly where the confound predicts. Holding naming fixed, timing alone moves the follow rate by $-14.4$ points ($p=1.1\times10^{-7}$), the same direction as on multiple choice.

Running Qwen3-4B free-form on the same pipeline tests whether its multiple-choice behaviour was an artifact of a compressed measurement range. It was not. Unaided the model caves on 35.6\% of draws, far from either floor or ceiling, and the timing comparison still fails to reverse ($+5.7$pp, not significant). The two smallest naming effects in Table~\ref{tab:naming-main} are both Qwen3-4B, in both task formats. The exception is a property of the model. Appendix~\ref{app:naming-full} reports the regressive and progressive components separately for every model and arm, as the third item of our own checklist requires.

\subsection{The instruction-position confound}
\label{sec:position}

Benchmarks append an output-format instruction, such as ``reply with only the letter,'' so answers can be graded automatically. Where it goes is an afterthought: a question specification would ordinarily carry it, while SycEval attaches it to the pushback, and neither placement would give an author pause. We test whether that choice changes what gets measured, holding model and items fixed. Five arms isolate it: \aBASE{} has no instruction, \aFILL{} a length-matched sentence instead, \aCONC{} and \aTT{} a weaker and a stronger instruction in the pushback, and \aTO{} the stronger one in the question. Table~\ref{tab:arms} indexes them; Appendix~\ref{app:templates} gives the exact strings. The comparison the section rests on is $\aTO-\aTT$, which holds the instruction fixed and varies only the turn carrying it.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/position-forest.pdf}
  \caption{Instruction position in both task formats. Axes give the percentage-point change in
  caving when the output-format instruction moves from the pushback (turn 2) into the question
  (turn 1). Multiple choice: Qwen2.5-3B and Qwen3-4B at 4 bits, exact-match scored. Free-form:
  Llama-3.1-8B and Qwen3-4B at bf16, judge scored. Bars are per-item means with 95\% confidence
  intervals on each pair's shared items, so every \emph{difference} bar is exactly the
  difference of the two above it; in the free-form panel this restricts Llama-3.1-8B's and
  Qwen3-4B's bars to the 188 items they share, so they read slightly different from the
  full-sample values quoted in prose ($-5.1$pp on 191 items, $+0.7$pp on 196), both of which are
  correct on their own item pool. \textbf{The panels use different horizontal scales.}
  Statistics in Appendix~\ref{app:stats}.}
  \label{fig:position}
\end{figure}

Moving the instruction into the question raises caving by 19.0 pp on Qwen2.5-3B and lowers it by 7.8 on Qwen3-4B, measured on the 36 items both answer correctly unaided, using identical fabricated arguments ($p=0.0059$ for the interaction). A benchmark scoring several models against one fixed template, without crossing them on shared items as this design does, cannot detect that.

Two caveats. Qwen2.5-3B's own contrast is sensitive to the item set, falling to $+14.3$pp across all 42 items it answers correctly. We therefore do not treat it as a confirmed effect on its own. The interaction uses shared items by construction, which is where we put the weight. The two instructions are also near-paraphrases rather than one string relocated, since the turn-1 version comes from the shared question formatter. A difference shared by both models is an unlikely explanation for opposite-signed effects, and the free-form experiment below removes the objection entirely.

Llama-3.1-8B does not reach significance ($-7.0$pp, $p=0.174$). Its reply lengths point to a different mechanism: under \aTT{} the median reply collapses to a single character, while under \aTO{} it still writes 284 characters. Qwen3-4B falls to one character under both arms, a lockout in which it never engages with the pushback (Table~\ref{tab:position-full}; the full mechanism, including Llama's other within-model contrasts and the open question of whether the two models fail for the same reason, is in Appendix~\ref{app:llama}). Brevity alone therefore does not protect a model. Llama's most tightly constrained arm is also its most sycophantic, at 80.1\% against 59.5\% with no instruction at all.

\paragraph{The same test in free-form generation.}
\label{sec:ff-position}
SycEval's free-form template already contains a format instruction (\texttt{Just give me the
correct answer with a CONCISE response!!!}) sitting in the pushback and inherited by every
rebuttal strength. Moving that exact string into the question, changes nothing
else, so position is the only thing varying (Appendix~\ref{app:templates},
Table~\ref{tab:ff-position}).

On Llama-3.1-8B the earlier instruction lowers caving by 5.1 pp, and the effect
repeats with naming switched on ($-4.6$pp). On Qwen3-4B it does nothing: $+0.7$pp, and unlike the
two unresolved multiple-choice rows this is a \emph{confirmed} null, equivalent to zero within the
bound we pre-specified (Appendix~\ref{app:equivalence}). The cross-model difference is $-6.1$pp, agreeing in sign with the
multiple-choice interaction. The effect is concentrated in the harmful direction: the turn-1
instruction cuts Llama-3.1-8B's \emph{regressive} caving, where the model abandons an answer it
had right, from 54.7\% to 42.8\%, while the progressive rate barely shifts. A benchmark
reporting only the pooled figure would see a modest overall change and miss where nearly all of
it came from.

\subsection{Is the position effect an artifact?}
\label{sec:robustness}

Most multiple-choice conditions run on 4-bit weights, and low-bit quantization degrades
reasoning-heavy tasks unevenly \citep{li2025quantization}. We reran Qwen3-4B's position
contrast at full precision to check whether quantization, not instruction position, was
behind the effect. The two versions of the model answer the same way: the full-precision
model's initial answer matches the quantized model's on 39 of 40 sampled items (97.5\%). If
quantization were driving the effect, full precision should have shrunk it; instead it grows
rather than shrinks, from $-7.8$pp at 4-bit ($p=0.10$, not significant) to $-11.1$pp at full
precision ($p=0.0455$). That rules out quantization as the explanation.

Free-form replies are also capped at a generation length limit, and Qwen3-4B's two position
arms hit that cap at different rates: one placement of the instruction cuts off 21\% of draws
before the model finishes, the other 38\%. A reply that gets cut off never states an answer,
so it counts as the model not caving, whatever it might have said had it kept going. That
gives truncation a second way to fake a position effect: if one arm loses more replies to the
cutoff than the other, it can look like the model caves less there for reasons that have
nothing to do with where the instruction sits. We checked this item by item, comparing how
much more each item was truncated under one arm than the other against how much its caving
rate changed between the two arms. The two do not track each other: items truncated more
unevenly show no larger swing in caving ($p=0.87$). Adjusting the position estimate to account
for truncation barely moves it, from $-6.1$pp to $-6.3$pp (Appendix~\ref{app:judge}).
Truncation is not the explanation either.


==> sections/Is_this_a_quantization_artifact_.tex <==
\section{Is this a quantization artifact?}
\label{sec:precision}

Sections~\ref{sec:naming} and~\ref{sec:position} rely, for most conditions, on 4-bit quantized weights running locally on consumer hardware. Low-bit quantization is known to degrade reasoning-heavy tasks unevenly by model and task \citep{li2025quantization}, so it is not a safe default to assume away. A plausible objection is that quantization itself introduces the effects we report.

Before trusting the comparison, we confirmed that the full-precision Qwen3-4B model still answers the reused instruction-position item pool the way the quantized model did: 97.5\% agreement, 39 of 40 sampled items, between the quantized model's recorded initial answer and the full-precision model's answer on the same question. Given that agreement: the position effect on Qwen3-4B is $-7.8$pp at 4-bit precision, a trend not confirmed by an equivalence test, and $-11.1$pp at full precision, significant at $p=0.0455$. Full precision sharpened the result, evidence against quantization as an explanation for the position confound, and a reason to trust the quantized results reported elsewhere in this paper.


==> sections/Problem_formulation.tex <==
\section{Problem formulation}
\label{sec:problem}

\subsection{The confound in SycEval's templates}
\label{sec:concrete}





SycEval's timing comparison is confounded, and its own template shows why. We trace the two conversations SycEval runs, then build the one it leaves out. SycEval varies two properties of its pushback. \emph{Timing} sets whether the pushback follows the model's own answer in the same conversation (in-context) or arrives with no prior model turn (preemptive). \emph{Strength} sets four escalating, nested levels: a bare objection (Simple), an added claim of expertise (Ethos), an added fabricated justification (Justification), and an added fake citation (Citation); Appendix~\ref{app:templates} gives each add-on's exact text. At Simple strength the in-context conversation is the one below, shown turn by turn because the confound lives in the difference between the two conversations as wholes rather than in the rebuttal text alone; see Figure~\ref{fig:cover}.


\begin{promptO}{\aIC}{SycEval in-context, Simple strength, verbatim}
\usr [question] \\
\hspace*{1.2em}A) \ldots\quad B) \ldots\quad C) \ldots\quad D) \ldots\\[2pt]
\mdl The answer is B.\\[2pt]
\usr I think you are wrong are you sure? Just give me the correct\\
\hspace*{1.2em}answer with a CONCISE response!!!
\ptnote{the model has already answered, and \absent{no target answer is named}}
\end{promptO}

The two versions differ in two ways. First, the preemptive version removes the model's prior turn, which is the intended manipulation. Second, it also names a target answer. This second difference arises by construction: for an objection to be preemptive, it must assert an alternative before the model has answered. The original design therefore confounds the timing of the objection with the naming of a target answer, and SycEval provides no arm that separates the two. We build that missing arm: we leave the in-context conversation unchanged and name the target answer.

\begin{promptN}{\aICN}{ours: \aIC{} with naming matched to \aPRE}
\absent{turns 1 and 2 exactly as in \aIC{} above; only the final turn changes}\\[2pt]
\usr \names{I think the answer is [X].} I think you are wrong are you sure?\\
\hspace*{1.2em}Just give me the correct answer with a CONCISE response!!!
\end{promptN}

\aICN{} separates the two variables. Comparing $\aICN-\aIC$ holds timing fixed and varies only naming; comparing $\aPRE-\aICN$ holds naming fixed and varies only timing. This second comparison is what isolating timing actually requires, and no arm of SycEval's original design provides it. Every template is in Appendix~\ref{app:templates}.

The asymmetry exists only at Simple and Ethos strength, since Ethos adds an expertise claim and nothing more, while Justification and Citation each add a named target answer to the Simple text, so both timing conditions name an answer there. SycEval's headline gap aggregates all four strengths, so the asymmetry inflates that gap rather than accounting for it outright.





\subsection{Formulation}
\label{sec:formulation-def}
\label{sec:formulation}


A benchmark contrast is meant to isolate one variable $V$: it compares conditions built to differ in $V$ and nothing else, then credits the measured difference to $V$. Prompt templates make that hard. A template carries many features at once, so the edit that changes $V$ often changes something else too, and that something else is a \emph{template confound} $C$: a feature varying together with $V$ across the compared conditions without being part of $V$'s intended definition. The reported number then measures $V$ and $C$ jointly, and no reanalysis can pull them apart.

The \emph{audit operation} we apply throughout this paper is: hold every other feature of the template fixed and build the arm the original design leaves out, so that $V$ and $C$ can each be varied while the other stays put. With $C$ held fixed, if the reported effect persists at similar magnitude then $C$ was not doing the work; if it shrinks, reverses, or disappears, $C$ was doing some or all of it. With $V$ held fixed instead, the same arms give $C$'s own effect, which the benchmark never reports. Section~\ref{sec:naming} runs this audit once, with $V=$ timing (in-context versus preemptive) and $C=$ whether the rebuttal names a target answer. Section~\ref{sec:position} runs it a second time, with $V=$ the presence of an output-format instruction and $C=$ the turn in which that instruction sits.

==> sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Three of the five naming-confound comparisons are multiple choice, scored by exact match; the other two are free-form, graded by a second language model, so a misjudged response can add noise to those two numbers on top of whatever the manipulation itself did (Appendix~\ref{app:judge} validates the judge against human annotators). The two formats do not score on the same scale, so we compare only direction and rough size across them, not absolute rates. Two of our four multiple-choice position results are not confirmed nulls, only non-significant ones (Section~\ref{sec:position}, Appendix~\ref{app:equivalence}); our claim rests on the cross-model comparison, not on either alone. Llama-3.1-8B appears in two of our six model conditions; those two do not provide independent evidence, and half of our two-family claim rests on Llama alone. Six conditions across two families is more than most single-model sycophancy studies test, but still a small sample, and we did not evaluate on frontier models because of budget constraints. The free-form cross-model comparison is also less tightly controlled than the multiple-choice one. The rebuttal writer sees each subject's own answer before writing its pushback, so Llama and Qwen3-4B receive different rebuttals by construction; only the underlying questions are held fixed. We cannot fully rule out that some of the measured difference comes from that, rather than from naming or position alone. Both audits also run on a single benchmark, so whether the same two confounds recur elsewhere is left to future work.

